Knowledge-Guided Data-Centric AI in Healthcare: Progress, Shortcomings, and Future Directions

The success of deep learning is largely due to the availability of large amounts of training data that cover a wide range of examples of a particular concept or meaning. In the field of medicine, having a diverse set of training data on a particular disease can lead to the development of a model that is able to accurately predict the disease. However, despite the potential benefits, there have not been significant advances in image-based diagnosis due to a lack of high-quality annotated data. This article highlights the importance of using a data-centric approach to improve the quality of data representations, particularly in cases where the available data is limited. To address this "small-data" issue, we discuss four methods for generating and aggregating training data: data augmentation, transfer learning, federated learning, and GANs (generative adversarial networks). We also propose the use of knowledge-guided GANs to incorporate domain knowledge in the training data generation process. With the recent progress in large pre-trained language models, we believe it is possible to acquire high-quality knowledge that can be used to improve the effectiveness of knowledge-guided generative methods.

==> fig_inception_1.tex <==
\tikzstyle{gnet_layer} = [draw=black, thick, minimum width=2.5cm, minimum height = 1.2cm, text width=2.5cm, align=center]
\begin{tikzpicture}[scale=.8]
\node[gnet_layer] (n1) {Feature Map \\ Concatenation};
\node[gnet_layer] (n2) [below of = n1,node distance=2cm]{3x3 \\ Convolutional Filters};
\node[gnet_layer] (n21) [left of = n2,node distance=3cm]{1x1 \\ Convolutional Filters};
\node[gnet_layer] (n22) [right of = n2,node distance=3cm]{5x5 \\ Convolutional Filters};
\node[gnet_layer] (n23) [right of = n22,node distance=3cm]{3x3 \\ Max Pooling};
\node[gnet_layer] (n3) [below of = n2,node distance=2cm]{ Previous \\ Feature Maps};
\draw[->,thick] (n3.north) -- (n2.south);
\draw[->,thick] (n3.north) -- (n21.south);
\draw[->,thick] (n3.north) -- (n22.south);
\draw[->,thick] (n3.north) -- (n23.south);
\draw[->,thick] (n2.north) -- (n1.south);
\draw[->,thick] (n21.north) -- (n1.south);
\draw[->,thick] (n22.north) -- (n1.south);
\draw[->,thick] (n23.north) -- (n1.south);
\end{tikzpicture}



==> fig_inception_2.tex <==
\tikzstyle{gnet_layer2} = [draw=black, thick, minimum width=2.5cm, minimum height = 1.2cm, text width=2.5cm, align=center]
\begin{tikzpicture}[scale=.8]
\node[gnet_layer2] (n1) {Feature Map \\ Concatenation};
\node[gnet_layer2] (n2) [below of = n1,node distance=2cm]{3x3 \\ Convolutional Filters};
\node[gnet_layer2] (n22) [right of = n2,node distance=3cm]{5x5 \\ Convolutional Filters};
\node[gnet_layer2] (n23) [right of = n22,node distance=3cm]{1x1 \\ Convolutional Filters};
\node[gnet_layer2] (n3) [below of = n2,node distance=1.5cm]{ 1x1 \\ Convolutional Filters};
\node[gnet_layer2] (n32) [right of = n3,node distance=3cm]{ 1x1 \\ Convolutional Filters};
\node[gnet_layer2] (n33) [right of = n32,node distance=3cm]{ 3x3 \\ Max Pooling};
\coordinate [below of=n2,node distance=0.8cm] (c1) {};
\node[gnet_layer2] (n31) [left of = c1,node distance=3cm]{1x1 \\ Convolutional Filters};
\node[gnet_layer2] (n4) [below of = n3,node distance=2cm]{Previous \\ Feature Maps};
\draw[->,thick] (n3.north) -- (n2.south);
\draw[->,thick] (n32.north) -- (n22.south);
\draw[->,thick] (n33.north) -- (n23.south);
\draw[->,thick] (n2.north) -- (n1.south);
\draw[->,thick] (n22.north) -- (n1.south);
\draw[->,thick] (n23.north) -- (n1.south);
\draw[->,thick] (n4.north) -- (n31.south);
\draw[->,thick] (n4.north) -- (n32.south);
\draw[->,thick] (n4.north) -- (n33.south);
\draw[->,thick] (n4.north) -- (n3.south);
\draw[->,thick] (n31.north) -- (n1.south);
\end{tikzpicture}


==> fig_residual_net.tex <==
\tikzstyle{res_layer} = [draw=black, thick, minimum width=3.5cm, minimum height = 0.7cm]
\begin{tikzpicture}
%\node[] (n0) {$x$};
\node[minimum size=0] (n0) {}; % invisible node
\coordinate [below of=n0,node distance=0.5cm] (n1) {}; % invisible node
\node[res_layer] (l1) [below of=n1,node distance=0.8cm]{parameter layer};
\node[res_layer] (l2) [below of=l1,node distance=1.5cm]{parameter layer};
\coordinate [right of=l1,node distance=2.5cm](ll1) ;
\coordinate [right of=l2,node distance=2.5cm](ll2);
\node[circle, draw=black,thick](c1)[below of=l2,node distance=1cm]{+} ;
\coordinate [below of=c1,node distance=1.0cm] (n2) {};
\draw[->,thick] (n0) -- node[auto,left] {f} (n1) -- (l1);
\draw[->,thick] (l1.south) --node[auto,right](p1) {ReLU}  (l2.north);
\draw[->,thick] (l2.south) -- (c1.north);
\draw[->,thick] (c1.south) -- node[auto,right] {ReLU} (n2)  ;
\draw[->,thick] (n1.east) to [bend left=90,out=90,in=90, distance=3.5cm] node[auto,right] {\begin{tabular}{c} f \\ identity  \end{tabular}} (c1.east);
\node[auto,left of=p1,node distance=3.0cm] {$\boldsymbol{M}_{r}(f)$};
\node[auto,left of=c1,node distance=1.5cm] {$\boldsymbol{M}_{r}(f)+f$ };
\end{tikzpicture}


